Efficient Multiparty Quantum Key Distribution over Quantum Networks

Multiparty quantum key distribution (QKD) is useful for many applications that involve secure communication or collaboration among multiple parties. While it can be achieved using pairwise QKD, a more efficient approach is to achieve it using multipartite entanglement distributed over quantum networks that connect the multiple parties. Existing studies on multipartite entanglement distribution, however, are not designed for multiparty QKD, and hence do not aim to maximize secret key generation rate. In this paper, we design efficient strategies for multiparty QKD over quantum networks. For 3-party QKD, we derive closed-form expressions for analyzing key distribution over quantum networks. We then use it to develop an efficient strategy for 3-party QKD by packing multiple stars that connect the 3 parties. For the general form of N-party QKD, we develop an approach that packs multiple trees to connect the N parties, while directly incorporating the estimated key rates on network paths. Extensive evaluation of our strategies, in both grid and random graphs, under a wide range of settings, demonstrates that our schemes achieve high key rate, which degrades gracefully when increasing the number of parties.

==> OldWriting.tex <==
\newpage
\mysection{Notation}
\subsection{Binary Entropy}
Let $H(p)$ denote the binary shannon entropy of $p$. That is \begin{equation*}
    H(p) = -[p\log_2{(p)} + (1-p)\log_2{(1-p)}] 
\end{equation*}

\subsection{Depolarizing Channel}
Typically the trace is omitted when defining the depolarizing channel since the trace of a density matrix of a state is always 1. However it is useful here since we will be distributing the depolarizing channel over partial states.
\begin{equation}
    \mathcal{E}(\rho) = \gamma \rho + (1 - \gamma) tr(\rho) \frac{\mathbb{I}}{2^n}
\end{equation}
Where $\gamma = \frac{4F - 1}{3}$, and $F$ is the fidelity of the state.
￼
\newpage
\mysection{Notation}
\subsection{Binary Entropy}
Let $H(p)$ denote the binary shannon entropy of $p$. That is \begin{equation*}
    H(p) = -[p\log_2{(p)} + (1-p)\log_2{(1-p)}] 
\end{equation*}
￼
\subsection{Depolarizing Channel}
Typically the trace is omitted when defining the depolarizing channel since the trace of a density matrix of a state is always 1. However it is useful here since we will be distributing the depolarizing channel over partial states.
\begin{equation}
    \mathcal{E}(\rho) = \gamma \rho + (1 - \gamma) tr(\rho) \frac{\mathbb{I}}{2^n}
\end{equation}
Where $\gamma = \frac{4F - 1}{3}$, and $F$ is the fidelity of the state.

\mysection{Stabilizer States}
A quantum state $\ket{\psi}$ is said to be stabilized by the operator $\mathcal{U}$ if the following equation holds:
\begin{equation*}
    \mathcal{U}\ket{\psi} = \ket{\psi}
\end{equation*}
The stabilizer formalism, as defined in \cite{nielsen00} allows us to describe quantum states by the operators that stabilize them. We can then use a subgroup of the Pauli group to describe a quantum state. For the n-qubit state $\ket{\psi}$ stabilized by the group $\mathcal{G}$ we can describe the density matrix, $\rho$, of $\ket{\psi}$ the following way.
\begin{equation*}
    \ketbra{\psi} = \rho = \frac{1}{2^n} \sum_{P\in \mathcal{G}}P
\end{equation*}
For example, the stabilizing group for the Bell state $\ket{\Phi^+}$ is $\mathcal{G} = \{II, XX, ZZ, -YY\}$, where $\mathcal{U}\mathcal{U}$ = $\mathcal{U}\otimes\mathcal{U}$. We can then describe the density matrix as follows
\begin{equation*}
    \ketbra{\Phi^+} = \frac{1}{4} \sum_{P\in \mathcal{G}}P = \frac{1}{4}(II + XX + ZZ - YY)
\end{equation*}
\mysection{Multiparty QKD}
The multiparty quantum key distribution protocol we will be using is from \cite{MP_QKD}, and is an N-partite variant of the BB84 protocol. 
\begin{itemize}
    \item[1.] $L$ $N$-GHZ states are distributed between the $N$ parties: $A$, $B_1,\ldots,B_{n-1}$
    \begin{equation*}
        \ket{\text{N-GHZ}} = \frac{1}{\sqrt{2}}(\ket{0}^{\otimes N} + \ket{1}^{\otimes N})
    \end{equation*}
    \item[2.] Each party measures in the $X$ or $Z$ basis, where the choice of measurement basis is predetermined using a fraction of the preshared key bits. A parameter $p$ denotes the fraction of $X$ vs. $Z$ basis measurement rounds. $m = Lp$ measurements are made in the $X$ basis, and $L-m$ measurements are made in the $Z$ basis. 
    \item[3.] Parameter Estimation:
    \begin{itemize}
        \item $Q_{AB_i}$ is the probability that parties $A$ and $B_i$ have different measurement outcomes when measuring in the $Z$ basis. 
        $\langle Z_A Z_{B_i}\rangle$ is the expectation of measuring in the $Z$ basis. 
        \begin{equation*}
            \langle Z_A Z_{B_i} \rangle = \text{Prob}[Z_A = Z_{B_i}] - \text{Prob}[Z_A \not= Z_{B_i}]
        \end{equation*}
        \begin{equation*}
            \langle Z_A Z_{B_i} \rangle = (1 - \text{Prob}[Z_A \neq Z_{B_i}]) - \text{Prob}[Z_A \not= Z_{B_i}]
        \end{equation*}
        \begin{equation*}
            \langle Z_A Z_{B_i} \rangle = 1 - 2* \text{Prob}[Z_A \not= Z_{B_i}]
        \end{equation*}
        \begin{equation*}
            \text{Prob}[Z_A \not= Z_{B_i}] = Q_{AB_i} = \frac{1 -  \langle Z_A Z_{B_i} \rangle}{2}
        \end{equation*}
        \item $Q_X$ is the probability that the total number of $\ket{-}$'s is odd when measuring in the X basis. Note that measuring a pure N-GHZ state in the X basis always yields an even number of $\ket{-}$'s.
        $\langle X^{\otimes N} \rangle$ is the expectation of measuring in the Z basis. 
        \begin{multline*}
            \langle X^{\otimes N} \rangle = \text{Prob[Even \# of $\ket{-}$'s measured]} \\ 
            - \text{Prob[Odd \# of $\ket{-}$'s measured]}
        \end{multline*}
        \begin{multline*}
            \langle X^{\otimes N} \rangle = (1 - \text{Prob[Odd \# of $\ket{-}$'s measured]}) \\ 
            - \text{Prob[Odd \# of $\ket{-}$'s measured]}
        \end{multline*}
        \begin{multline*}
            \langle X^{\otimes N} \rangle = 1 - 2*\text{Prob[Odd \# of $\ket{-}$'s measured]}
        \end{multline*}
        \begin{multline*}
            \text{Prob[Odd \# of $\ket{-}$'s measured]} = Q_X \\ = \frac{1 - \langle X^{\otimes N} \rangle}{2}
        \end{multline*}
    \end{itemize}
\end{itemize}
\cite{MP_QKD} provides only the finite keyrate equation. However, their equation can easily be extended to the asymptotic case for the depolarizing noise model.
\begin{equation} \label{eq:keyrate}
    \text{Keyrate} = R  [1 - H(Q_X) - \max_i H(Q_{AB_i})]
\end{equation}
Where $R$ is the entanglement distribution rate. 

By computing the expectations directly from our noisy N-GHZ state, we can obtain equations for Q$_X$ and Q$_{AB_i}$ dependent on our $\gamma$ values.
\begin{equation} \label{eq:Q_X}
    Q_X = \frac{1 - \langle X^{\otimes N} \rangle}{2} = \frac{1 - \prod_i \gamma_i}{2}
\end{equation}
\begin{equation} \label{eq:Q_AB_i}
    Q_{AB_i} = \frac{1 - \langle Z_A Z_{B_i}\rangle}{2} = \frac{1 - \gamma_1 \gamma_i}{2}
\end{equation}
H($Q_{AB_i}$) is maximized when $Q_{AB_i} = \frac{1}{2}$. We know that $\gamma_i \geq \frac{1}{3}$, since when $\gamma_i < \frac{1}{3}$ we have $F_i < \frac{1}{2}$ and entanglement no longer exists. Thus $\gamma_1\gamma_i \geq \frac{1}{9}$ and $Q_{AB_i} \leq \frac{4}{9} $. The maximum value of $Q_{AB_i}$ is achieved with the smallest $\gamma_i$. 
\begin{equation} \label{eq:keyrate2}
    \text{Keyrate} = R * \left[1 - H\left(\frac{1 - \prod_i \gamma_i}{2}\right) - H\left(\min_i \frac{1 - \gamma_1 \gamma_i}{2}\right)\right]
\end{equation}



\mysection{Keyrate from Fidelity of N-GHZ}
Consider three Bell pairs, each with a depolarising channel acting on them, with fidelity $F_i$ = $\frac{3\gamma_i + 1}{4}$. Each of these can be represented as a Werner state.
\begin{equation}
    \mathcal{E}(\ketbra{\Phi^+}) = \gamma_i \ketbra{\Phi^+} + (1-\gamma_i) \frac{\mathbb{I}}{4}
\end{equation}

The stabilizer representation of $\mathcal{E}(\ketbra{\Phi^+})$ is
\begin{equation}
    \mathcal{E}(\ketbra{\Phi^+}) = \gamma_i \frac{1}{4} \sum_{P \in \mathcal{G}}P + (1-\gamma_i) \frac{\mathbb{I}}{4} 
\end{equation}
Where $\mathcal{G} = \{II, XX, ZZ, -YY\}$.

 As shown in Figure 1, the depolarizing noise can be modeled on the outer qubits rather than the center qubit. This is because applying the depolarizing noise to the first qubit in a Bell pair is identical to applying the depolarizing noise to the second qubit. Then a perfect N-GHZ measurement can be made on the center qubits, and after local correction, the final noisy N-GHZ state can be represented by applying the depolarizing channel to each of the remaining qubits making up the perfect N-GHZ state.


 Note that the stabilizing group for the 3-GHZ state is $\mathcal{G}=\{III, XXX, IZZ, ZZI, ZIZ, -YYX, -XYY, -YXY\}$.
 
\begin{multline}
    %\mathcal{E}_1(\rho_1) \otimes \mathcal{E}_2(\rho_2) \otimes \mathcal{E}_3(\rho_3) 
    \rho = \mathcal{E}_1(\mathcal{E}_2(\mathcal{E}_3 (\ketbra{\text{3-GHZ}}))) 
    \\ = \mathcal{E}_1(\mathcal{E}_2(\mathcal{E}_3 (\frac{1}{8} \sum_{P \in \mathcal{G}} P)
     = \frac{1}{8} \sum_{P \in \mathcal{G}} \mathcal{E}_1(\mathcal{E}_2(\mathcal{E}_3(P)))
    \\ = \frac{1}{8} * (III + \gamma_1 \gamma_2 \gamma_3 XXX  + \gamma_2 \gamma_3 IZZ + \gamma_1 \gamma_2 ZZI \\ + \gamma_1 \gamma_3 ZIZ - \gamma_1 \gamma_2 \gamma_3 YYX 
     -\gamma_1 \gamma_2 \gamma_3 XYY - \gamma_1 \gamma_2 \gamma_3 YXY)
\end{multline}

The fidelity of this state can be expressed as \begin{multline}
    F = tr(\rho \ketbra{\text{3-GHZ}}) \\ = tr(\frac{1}{8}(III + \gamma_1 \gamma_2 \gamma_3 XXX  + \gamma_2 \gamma_3 IZZ + \gamma_1 \gamma_2 ZZI \\ + \gamma_1 \gamma_3 ZIZ - \gamma_1 \gamma_2 \gamma_3 YYX 
     -\gamma_1 \gamma_2 \gamma_3 XYY - \gamma_1 \gamma_2 \gamma_3 YXY)\\ \frac{1}{8}(III + XXX + IZZ + ZZI + ZIZ - YYX - XYY - YXY))
\end{multline}
\begin{equation}
    F = \frac{1}{8} * (1 + 4 \gamma_1 \gamma_2 \gamma_3 + \gamma_1 \gamma_2 + \gamma_2 \gamma_3 + \gamma_1 \gamma_3)
\end{equation}

This becomes more tedious to compute as $N$ increases. However for making routing decisions we only need to compute the keyrate, which depends on $Q_X$ and $Q_{AB_i}$ and can easily be computed as seen in \eqref{eq:Q_X} and \eqref{eq:Q_AB_i}.

\begin{figure}
    \centering
    \begin{tikzpicture}

    % Left Diagram
    \coordinate (A1) at (4, 5.5);
    \coordinate (B1) at (2.5, 3);
    \coordinate (C1) at (5.5, 3);
    \coordinate (A2) at (4, 4.2);
    \coordinate (B2) at (3.8, 3.9);
    \coordinate (C2) at (4.2, 3.9);
    
    \filldraw (A1) circle (0.05);
    \filldraw (B1) circle (0.05);
    \filldraw (C1) circle (0.05);
    \filldraw (A2) circle (0.05);
    \filldraw (B2) circle (0.05);
    \filldraw (C2) circle (0.05);

    \draw (3.9, 4.1) rectangle (4.1, 4.3);
    \draw (3.7, 3.8) rectangle (3.9, 4.0);
    \draw (4.1, 3.8) rectangle (4.3, 4.0);

    \draw (A1)--(A2);
    \draw (B1)--(B2);
    \draw (C1)--(C2);
    
    \draw (4,4) circle (0.5);

    % Equiv
    \draw (6, 4.1) -- (6.2, 4.1);
    \draw (6, 4) -- (6.2, 4);
    \draw (6, 3.9) -- (6.2, 3.9);

    % Right Diagram
    \coordinate (A1') at (8, 5.5);
    \coordinate (B1') at (6.5, 3);
    \coordinate (C1') at (9.5, 3);
    \coordinate (A2') at (8, 4.2);
    \coordinate (B2') at (7.8, 3.9);
    \coordinate (C2') at (8.2, 3.9);
    
    \filldraw (A1') circle (0.05);
    \filldraw (B1') circle (0.05);
    \filldraw (C1') circle (0.05);
    \filldraw (A2') circle (0.05);
    \filldraw (B2') circle (0.05);
    \filldraw (C2') circle (0.05);

    \draw (7.9, 5.4) rectangle (8.1, 5.6);
    \draw (6.4, 2.9) rectangle (6.6, 3.1);
    \draw (9.4, 2.9) rectangle (9.6, 3.1);

    \draw (A1')--(A2');
    \draw (B1')--(B2');
    \draw (C1')--(C2');
    
    \draw (8,4) circle (0.5);
    
\end{tikzpicture}
    \caption{The depolarising noise is shown as a box on each qubit. Modeling with the noise affecting the qubits in the center node is identical to modeling the noise such that it affects the qubits in the terminal nodes.}
    \label{fig:enter-label}
\end{figure}

\subsection{Minimum Fidelity}
What is the minimum required fidelity required to achieve a positive keyrate? In \eqref{eq:keyrate2} we see that in order to have a positive keyrate we must have
\begin{equation*}
    H\left(\frac{1 - \prod_i \gamma_i}{2}\right) + H\left(\min_i \frac{1 - \gamma_1 \gamma_i}{2}\right) < 1
\end{equation*}
We also know that H(Q$_X$) $\geq$ H(Q$_{AB_i}$), and thus we must have H(Q$_{AB_i}$) $< \frac{1}{2}$. \st{The maximum of H(Q$_X$) is achieved when all $\gamma_i$'s are equal, since the other $\gamma$ values cannot take a lower value than the $\gamma_i$ in Q$_{AB_i}$. 
Assuming all $\gamma_i$'s are equal, and subjected to H(Q$_{AB_i}$) $< \frac{1}{2}$, we find that $\gamma_i \geq 0.943398$, implying the fidelity restriction on each path to the center being F $> 0.9575$.}

\subsection{Entanglement Distribution}
Prior to executing the QKD protocol, users must posess part of an $N$-GHZ state. Distributing these states in a network settings is a difficult task and has been previously studied in \cite{Bugalho_2023, Sutcliffe_2023, Meignant_2019}. The optimal way to distribute an $N$-GHZ state is by solving the Steiner tree problem \cite{Meignant_2019}. However solving the steiner tree problem is an NP-hard, which makes this non-trivial. However by simplifying the problem to distributing a 3-GHZ state, the optimal solution is to find the shortest star, a much more tractable problem \cite{Bugalho_2023}.

\subsection{Routing Algorithm}

\section{Simulation}
\begin{itemize}
    \item \textit{Trials}: How many times to repeat the simulation
    \item \textit{Iterations}: How many timesteps in the simulation
    \item \textit{P}: Probability of link level entanglement success
    \item \textit{Q}: Probability of entanglement swapping success
    \item \textit{Snapshot}: A snapshot of the graph is what the graph looks like after link level entanglement. It is a subgraph of the initial graph
    \item \textit{Dynamic Routing}: The routing algorithm is ran at each timestep for a snapshot of the graph. Link level entanglement is assumed to be global knowledge. If a star is found then the QKD protocol is ran.
    \item \textit{Fixed Routing}: The routing algorithm is ran once before any iterations occur. The optimal star based on keyrate is determined and during each timestep if the link level entanglement for each path forming the star is successful then the QKD protocol is ran. 
    \item \textit{Avg Keyrate}:
    Each center computes $Q_X$ and $Q_{AB_i}$ and plugs them into the keyrate equation. Then a weighted average of the keyrates from each center is taken.
    \item \textit{Pooled Keyrate}:
    Each center pools all of their raw keybits, then $Q_X$ and $Q_{AB_i}$ are sampled from the pool to compute the keyrate.
\end{itemize}

\sam{Need to mention edge case where terminal creates local entanglement (fid=1)}
\\
\sam{Mention that for creating multiparty key from pairwise keys we have K$_{AB}$ K$_{BC}$ then K$_{ABC}$ has length of the min of both. B will encrypt the smaller key and send it to the other party and then all 3 use that key. Should be able to find trusted node citation in QKD survey paper...}
\section{Results}

==> n-GHZ-dist.tex <==
\section{Obtain key rate for n-Party in Quantum Network}
%n-GHZ Distribution; 

This can be merged with \S\ref{sec:routing}. 
3-party: optimal star

Key rate expression 

n-party: Given a tree, how to obtain key rate


==> routing.tex <==
\section{Routing for n-party QKD} \label{sec:routing}

Main idea: stack trees 

3-party: find optimal centers (in terms of maximizing key rate)

n-party: find Steiner tree using approximation algorithm  


